Crosslingual Generalization through Multitask Finetuning

Multitask prompted finetuning (MTF) has been shown to help large language models generalize to new tasks in a zero-shot setting, but so far explorations of MTF have focused on English data and models. We apply MTF to the pretrained multilingual BLOOM and mT5 model families to produce finetuned variants called BLOOMZ and mT0. We find finetuning large multilingual language models on English tasks with English prompts allows for task generalization to non-English languages that appear only in the pretraining corpus. Finetuning on multilingual tasks with English prompts further improves performance on English and non-English tasks leading to various state-of-the-art zero-shot results. We also investigate finetuning on multilingual tasks with prompts that have been machine-translated from English to match the language of each dataset. We find training on these machine-translated prompts leads to better performance on human-written prompts in the respective languages. Surprisingly, we find models are capable of zero-shot generalization to tasks in languages they have never intentionally seen. We conjecture that the models are learning higher-level capabilities that are both task- and language-agnostic. In addition, we introduce xP3, a composite of supervised datasets in 46 languages with English and machine-translated prompts. Our code, datasets and models are freely available at https://github.com/bigscience-workshop/xmtf.

==> authors.tex <==
\begin{comment}
{\footnotesize YOURNAME } \\ {\footnotesize YOUR AFFILIATION } \And
{\footnotesize Niklas Muennighoff } \\ {\footnotesize Hugging Face } \And
{\footnotesize Thomas Wang} \\ {\footnotesize Hugging Face} \And
{\footnotesize Lintang Sutawika } \\ {\footnotesize Datasaur.ai } \And
{\footnotesize Adam Roberts} \\ {\footnotesize Google Research, Brain Team} \And
{\footnotesize Teven Le Scao} \\ {\footnotesize Hugging Face} \And
{\footnotesize M Saiful Bari} \\ {\footnotesize NTU, Singapore} \And
{\footnotesize Sheng Shen} \\ {\footnotesize UC Berkeley} \And 
{\footnotesize Zheng-Xin Yong} \\ {\footnotesize Brown University} \And
{\footnotesize Hailey Schoelkopf} \\ {\footnotesize EleutherAI, Yale University} \And
{\footnotesize Dragomir Radev} \\ {\footnotesize Yale University (ok to leave me out)} \And
{\footnotesize Alham Fikri Aji} \\ {\footnotesize } \And
{\footnotesize Samuel Albanie} \\ {\footnotesize University of Cambridge} \And 
{\footnotesize Albert Webson} \\ {\footnotesize Brown University} \And
{\footnotesize Colin Raffel } \\ {\footnotesize Hugging Face } \And
\end{comment}


Niklas Muennighoff$^{1}$
\quad Thomas Wang$^1$ 
\quad Lintang Sutawika$^{2,3}$ 
\quad Adam Roberts$^4$
\quad Stella Biderman$^{3,5}$\\
\bf \quad Teven Le Scao$^1$
\bf \quad M Saiful Bari$^6$ 
\bf \quad Sheng Shen$^7$ 
\bf \quad Zheng-Xin Yong$^8$
\bf \quad Hailey Schoelkopf $^{3,9}$\\
\bf \quad Xiangru Tang $^9$ 
\bf \quad Dragomir Radev$^9$ 
\bf \quad Alham Fikri Aji$^{10}$
\bf \quad Khalid Almubarak$^{11}$\\
\bf \quad Samuel Albanie$^{12}$
\bf \quad Zaid Alyafeai$^{13}$
\bf \quad Albert Webson$^8$
\bf \quad Edward Raff$^{5}$
\bf \quad Colin Raffel$^1$ \\
  $^1$Hugging Face \quad
  $^2$Datasaur.ai \quad
  $^3$EleutherAI \quad
  $^4$Google Research, Brain Team \quad
  $^5$Booz Allen Hamilton \quad\\
  $^6$Nanyang Technological University \quad
  $^7$ UC Berkeley \quad
  $^8$ Brown University \quad \\
  $^9$ Yale University \quad
  $^{10}$ MBZUAI \quad  
  $^{11}$ PSAU \quad
  $^{12}$ University of Cambridge 
  $^{13}$ KFUPM\\
  {\tt niklas@hf.co}
